AutoMAS: A Generic Multi-Agent System for Algorithm Self-Adaptation in Wireless Networks

The wireless communication environment has the characteristic of strong dynamics. Conventional wireless networks operate based on the static rules with predefined algorithms, lacking the self-adaptation ability. The rapid development of artificial intelligence (AI) provides a possibility for wireless networks to become more intelligent and fully automated. As such, we plan to integrate the cognitive capability and high intelligence of the emerging AI agents into wireless networks. In this work, we propose AutoMAS, a generic multi-agent system which can autonomously select the most suitable wireless optimization algorithm according to the dynamic wireless environment. Our AutoMAS combines theoretically guaranteed wireless algorithms with agents' perception ability, thereby providing sounder solutions to complex tasks no matter how the environment changes. As an example, we conduct a case study on the classical channel estimation problem, where the mobile user moves in diverse environments with different channel propagation characteristics. Simulation results demonstrate that our AutoMAS can guarantee the highest accuracy in changing scenarios. Similarly, our AutoMAS can be generalized to autonomously handle various tasks in 6G wireless networks with high accuracy.

==> trash.tex <==
\noindent\textbf{Phase 1: Supervisor Pre-processing}
%如图2所示，Supervisor接收到任务和观测，在agent pool中挑选算法选择师和code agent来处理任务，分别负责算法挑选与代码执行。
%supervisor为这两个设计了algorithm selector为code agent提供算法设计，code agent执行代码并在性能阈值下进行refine的闭环流程。
%该智能负责完成AnoMAS工作流设计，实现算法调整的自动化。
As shown in Fig. \ref{fig_example}, the Supervisor receives the task specification and environmental observations, then activates an Algorithm Selector and a Code Agent to handle strategy design and implementation, respectively. 
%
The Algorithm Selector proposes an estimation strategy, which the Code Agent executes and evaluates; the resulting performance feedback is relayed back to the Selector for iterative, cross-agent refinement.
%
By coordinating role activation and workflow orchestration, the Supervisor fully automates and streamlines the dynamic adaptation of channel estimation algorithms.
\noindent\textbf{Phase 2: Algorithm Design}
\begin{itemize}
    \item \textit{0-step Action (Think)}:  
    The Algorithm Selector analyzes the rural scenario to infer channel characteristics.  
    
    \textit{Observation}: High-frequency propagation (60 GHz) in open terrain suggests a sparse multipath profile.
    
    \item \textit{1-step Action (Algorithm Select)}:  
    Chooses the Iterative Shrinkage-Thresholding Algorithm (ISTA) based on:
    \begin{itemize}
        \item \textit{Environmental Fit}: ISTA exploits channel sparsity, matching the inferred multipath profile.  
        \item \textit{System Constraints}: Its iterative design balances estimation accuracy with computational overhead.  
        \item \textit{Operational Cost}: Requires no statical or training data.  
    \end{itemize}

    \textit{Observation}: Selected algorithm: Compressed sensing via ISTA.
    
    \item \textit{2-step Action (Finish)}:  
    Finalizes the algorithm specification, detailing sparse-domain formulation, ISTA iteration steps, parameter settings, and validation criteria.  
    \textit{Observation}: Complete workflow prompt prepared (see Appendix XX).
\end{itemize}


% Finalizes mathematical formulation with sparse domain transformation $\mathbf{x}=\mathbf{Fh}$ and iteration rule:  
% \begin{equation}  
% \mathbf{x}^{(k+1)} = \mathcal{S}_{\lambda\mu}\left(\mathbf{x}^{(k)} - \mu\mathbf{A}^H(\mathbf{A}\mathbf{x}^{(k)}-\mathbf{y})\right).
% \end{equation}  
% \begin{itemize}  
%     \item Adaptive step size $\mu = 1/\|\mathbf{A}^H\mathbf{A}\|_2$  
%     \item Noise-dependent $\lambda = \sigma\sqrt{2\log N}$ ($N=64$)  
% \end{itemize}  
\noindent\textbf{Phase 3: Code Generation}
\begin{itemize}
    \item \textit{0-step Action (Think)}:  
    The Code Agent outlines the implementation strategy for ISTA-based channel estimation.  
    \textit{Observation}: Establishes the functional flow of the algorithm, maps environmental descriptors to code variables (e.g., SNR, antenna count), and outlines the structure of the test module.
    
    \item \textit{1-step Action (Execute Code)}:  
    Produces and runs the ISTA code, featuring:
    \begin{itemize}
        \item Soft-thresholding adapted for complex-valued channel coefficients  
        \item Automated loading of \texttt{h\_test\_rural.mat} test data  
        \item NMSE evaluation module integrated into the test pipeline  
    \end{itemize}
    \textit{Observation}: Code executed successfully with output:  
    \begin{verbatim}
    [Result] NMSE: -19.76 dB
    \end{verbatim}
    
    \item \textit{2-step Action (Finish)}:  
    Consolidates channel estimation results and evaluation metrics.  
    \textit{Observation}: Performance report compiled and delivered to the Supervisor.
\end{itemize}


\noindent \textbf{Cross-Agent Refinement}

%Code agent在输出NMSE后会根据结果来判断是否进行refine loop。
%判断的基准为LS的NMSE，若性能比它差，则进入refine。
%code agent将结果重新输入至algorithm selector，让其verifies sparsity assumption是否合理，判断是否需要更改正则项，或是重新挑选算法。
%这个Refine loop的检验机制增强了输出的可靠性。
The Code Agent triggers the refine loop when the achieved NMSE underperforms the LS benchmark.
%
Upon detecting such cases, it packages estimated testing channel and performance metrics into diagnostic reports, which are routed back to the Algorithm Selector for joint analysis.
%
The Algorithm Selector then verifies the sparsity assumption validity through statistical indicators, subsequently deciding whether to adjust regularization parameters or initiate alternative algorithm selection.
%
This closed-loop validation enhances output reliability by dynamically aligning theoretical assumptions with practical channel characteristics
